Free-DyGS: Camera-Pose-Free Scene Reconstruction for Dynamic Surgical Videos with Gaussian Splatting

High-fidelity reconstruction of surgical scene is a fundamentally crucial task to support many applications, such as intra-operative navigation and surgical education. However, most existing methods assume the ideal surgical scenarios - either focus on dynamic reconstruction with deforming tissue yet assuming a given fixed camera pose, or allow endoscope movement yet reconstructing the static scenes. In this paper, we target at a more realistic yet challenging setup - free-pose reconstruction with a moving camera for highly dynamic surgical scenes. Meanwhile, we take the first step to introduce Gaussian Splitting (GS) technique to tackle this challenging setting and propose a novel GS-based framework for fast reconstruction, termed \textit{Free-DyGS}. Concretely, our model embraces a novel scene initialization in which a pre-trained Sparse Gaussian Regressor (SGR) can efficiently parameterize the initial attributes. For each subsequent frame, we propose to jointly optimize the deformation model and 6D camera poses in a frame-by-frame manner, easing training given the limited deformation differences between consecutive frames. A Scene Expansion scheme is followed to expand the GS model for the unseen regions introduced by the moving camera. Moreover, the framework is equipped with a novel Retrospective Deformation Recapitulation (RDR) strategy to preserve the entire-clip deformations throughout the frame-by-frame training scheme. The efficacy of the proposed Free-DyGS is substantiated through extensive experiments on two datasets: StereoMIS and Hamlyn datasets. The experimental outcomes underscore that Free-DyGS surpasses other advanced methods in both rendering accuracy and efficiency. Code will be available.

==> method_v0.tex <==
\section{Methods}
%这里加一段总述 - 整体介绍一些proposed framework, 一步一步是怎么进行的，可以参考[2024TMI]Video-Instrument_Synergistic_Network_for_Referring_Video_Instrument_Segmentation_in_Robotic_Surgery 这篇paper的对应段落，有点类似你现在写在intro的那段，不过记得highlight novelty （也就是设计了什么）；也可以参考硕崛miccai pipeline那里

\subsection{Preliminaries for 3D Gaussian splatting}
%Our method is based on the Gaussian splatting. It is a fast 3D reconstruction method for static scenes, where a set of generalized Gaussian point clouds $\mathcal{G}$ are used to map the scene. Each Gaussian ${G}_n$ contains attributes of mean $\bm{\mu}_n$, scale $\mathbf{s}_n$, and quaternions-described rotation $\mathbf{r}_n$ to define its position in the world coordinate system and the shape, which can be expressed as

Our method is based on Gaussian splatting, a fast 3D reconstruction technique for static scenes. It utilizes a collection of generalized Gaussian point clouds to represent the scene. Each Gaussian, denoted as \( G_n \), encompasses several attributes: the mean vector \( \bm{\mu}_n \), the scale vector \( \mathbf{s}_n \), and a quaternion \( \mathbf{r}_n \) that describes its orientation. These attributes collectively define the position within the world coordinate system and the geometric shape, which can be mathematically expressed as

\[G_n(\mathbf{x})=\exp{\left(-\frac{1}{2}(\mathbf{x}-\bm{\mu}_n)^T\mathbf{\Sigma}_n^{-1}(\mathbf{x}-\bm{\mu}_n)\right)}\]

\[\mathbf{\Sigma}_n=\mathbf{R}_n\mathbf{S}_n\mathbf{S}_n^T\mathbf{R}_n^T\]
where $\mathbf{\Sigma}_n$ is the covariance matrix, $\mathbf{S}_n$ the diagonal matrix of the scaling vector $\mathbf{s}_n$
, and $\mathbf{R}_n$ is the rotation matrix derived from the quaternions $\mathbf{r}_n$.

Given a camera pose matrix $\mathbf{T}$, a 3D Gaussian in the world coordinate system can be projected onto the image plane as 2D Gaussian $G^{2D}$ with the position and covariance matrix of

\begin{equation}
\label{eq:proj}
    \bm{\mu}^{2D}=\pi(\bm{\mu}^{C})=\pi(\mathbf{T}\bm{\mu}), \mathbf{\Sigma}^{2D}=\mathbf{J}\mathbf{W}\mathbf{\Sigma}\mathbf{W}^T\mathbf{J}^T
\end{equation}

where $\pi$ denotes the projection function, $\bm{\mu}^{C}$ is the Gaussian center in the camera coordinates, $\mathbf{J}$ is the Jacobian of the affine approximation of the projective transformation, and $\mathbf{W}$ represents the rotational component of the camera pose matrix $\mathbf{T}$. 

%Meanwhile, Gaussian ${G}_n$ is also associated with an opacity $\alpha_n$ and a learnable color $\mathbf{c}_n$ which is described by spherical harmonics parameters. The color of a pixel in the rendered image can be formulated as an alpha blending of all the Gaussians covering that pixel. In a similar way, the depth corresponding to the rendered image can also be obtained.

Furthermore, Gaussian ${G}_n$ is also characterized by an opacity value  $\alpha_n$ and a learnable color $\mathbf{c}_n$ described by spherical harmonics parameters. The pixel color in the rendered image is determined through an $\alpha$-blending process that considers all the Gaussians that overlap the pixel's location. Similarly, the depth information for the rendered image can be derived by applying the alpha blending to the depth values associated with each Gaussian:
\[\mathbf{C}(x)=\sum_n^N{\mathbf{c}_n\alpha_nG_n^{2D}(x)\prod_m^{n-1}({1-\alpha_mG_n^{2D}(x)})}\]
\[d(x)=\sum_n^N{[\mathbf{T}\bm{\mu}_n]_\text{z}\alpha_nG_n^{2D}(x)\prod_m^{n-1}{(1-\alpha_mG_n^{2D}(x))}}\]
It makes the rendering process differentiable, and the attributes of the 3D Gaussian can be gradually optimized through backward propagation of the gradient flow. 

\subsection{Camera pose optimization }
The training of Gaussians and high-quality scene reconstruction heavily depends on the precision of the camera poses. Thanks to the differentiable Gaussian splatting process, the camera pose can also be optimized by utilizing the derivatives of terms in Eq. (\ref{eq:proj}) with respect to the camera pose $\mathbf{T}$. 
We utilize an efficient derivatives calculation method\cite{yugay2023gaussian}, where the Jacobian of the camera position is described as derivatives on the manifold,


\begin{equation}
    \begin{aligned}
\frac{\partial \boldsymbol{\mu}^{2D}}{\partial \mathbf{T}} & =\frac{\partial \boldsymbol{\mu}^{2D}}{\partial \boldsymbol{\mu}^{C}} \frac{\mathcal{D} \boldsymbol{\mu}^{C}}{\mathcal{D} \mathbf{T}} \\
\frac{\partial \boldsymbol{\Sigma}^{2D}}{\partial \mathbf{T}} & =\frac{\partial \boldsymbol{\Sigma}^{2D}}{\partial \mathbf{J}} \frac{\partial \mathbf{J}}{\partial \boldsymbol{\mu}^{C}} \frac{\mathcal{D} \boldsymbol{\mu}^{C}}{\mathcal{D} \mathbf{T}}+\frac{\partial \boldsymbol{\Sigma}^{2D}}{\partial \mathbf{W}} \frac{\mathcal{D} \mathbf{W}}{\mathcal{D} \mathbf{T}} \\
\frac{\mathcal{D} \boldsymbol{\mu}^{C}}{\mathcal{D} \mathbf{T}} & =\left[\begin{array}{ll}
\boldsymbol{I} & -\boldsymbol{\mu}^{C\times}
\end{array}\right] \\
\frac{\mathcal{D} \mathbf{W}}{\mathcal{D} \mathbf{T}} & =\left[\begin{array}{cc}
\mathbf{0} & -\mathbf{W}_{:, 1}^{\times} \\
\mathbf{0} & -\mathbf{W}_{:, 2}^{\times} \\
\mathbf{0} & -\mathbf{W}_{:, 3}^{\times}
\end{array}\right]
\end{aligned}
\end{equation}
where and $\mathbf{W}_{:,i}$ refers the the $i$th column of the matrix $\mathbf{W}$ and $\mathbf{W}_{:,i}^{\times}$ denotes the skew symmetric matrix of the vector $\mathbf{W}_{:,i}$.

\subsection{Pose-free Dynamic scene reconstruction}
\label{sec:3.3}


\begin{figure*}[t]
	\centering
	\includegraphics[width=0.9\textwidth]{figs/method.pdf}
	\vspace{-3mm}
	\caption{Illustration of our Free-DyGS framework. Given an endoscopy video, we estimate the camera pose and reconstruct the scene frame-by-frame. Our approach is structured into four main phases: (a)Scene Initialization: We employ a pre-trained Gaussian Regression Network (GRN) to predict appropriate Gaussian attributes from the RGB image and depth map of the initial frame. These Gaussians are then translated into the world coordinate system using the initial camera pose \(\mathbf{T}_0\), thereby establishing the initial reconstruction. (b) Joint Learning: At each time instance \(t_i\), we deform the previous Gaussian model \(\mathcal{G}_{i-1}\) and iteratively optimize the camera pose and deformation model by comparing the current frame with rendering outputs. Additionally, an invisible mask \(M^{\text{ivsb}}_i\) is derived by thresholding the rendered opacity, which delineates the region for expansion. (c) Scene Expansion: In this phase, the corresponding additional Gaussians \(\mathcal{G}^{\text{add}}_i\) are generated using the GRN. These are then merged to form the updated model \(\mathcal{G}_i\). (d) Retrospective Learning: The final phase focuses on refining the learned deformation model. This is accomplished by retraining the model on a selection of historical frames to enhance accuracy and robustness.}

	\label{fig:method}
	\vspace{-5mm}
\end{figure*}

As depicted in  Fig. \ref{fig:method}, the proposed method primarily comprises four stages: scene initialization, camera pose estimation, scene expansion, and deformation retrospective learning. Both the scene initialization and scene expansion stages incorporate an efficient generalizable Gaussian generation technique. Once pre-trained, this module ensures fast and high-quality Gaussian parameterization for novel scenes. The specifics are detailed in Sec. \ref{sec:3.4}. 

\subsubsection{Scene initialization}
The first frame is token for the scene initialization and Gaussians are generated from pixels. Specifically, the GRN outputs the Gaussian parameters and positions on the camera coordinate system with the original image $I_0$ and the depth map $D_0$ as input. 
They are then further transformed to the word coordinate system with the initial camera pose \( \mathbf{T}_0 \). Thus, the initial Gaussians $\mathcal{G}_0$ can be described with a defined operator $\mathbb{G}$ which generates Gaussians from the parameters and the camera pose: 

\begin{equation}
    \mathcal{G}_0=\mathbb{G}(GRN(I_0, D_0), \mathbf{T}_0)
\end{equation}

\subsubsection{Jointly learning camera pose and scene deformation}
In the endoscopy scene, tissue deformation and camera moving occur concurrently over time. It would be hard to accurately recover the camera trajectory from a static scene. Consequently, when estimating the camera pose, we simultaneously incorporate camera tracking and scene deformation when training. At time $t_i$, both the camera pose and deformation model are jointly updated based on the previously learned Gaussians $\mathcal{G}_{i-1}$. This iterative process is executed \( k \) times to gradually refine the camera pose, evolving from the initial pose \( \mathbf{T}^0_i \) to the refined one \( \mathbf{T}^k_i \). In our approach,  \( \mathbf{T}^0_i \)  is calculated based on the previous estimation results $\{\mathbf{T}^k_{i-j}|j=1,2,...,6\}$. Following the operation in \cite{wang2023bad}, \ym{a velocity calculated in the Lie algebra domain is used:}
\begin{equation}
    \mathbf{T}^0_i=\mathbf{T}^k_{i-1}\exp (\sum_{j=1}^3(\log\mathbf{T}^k_{i-j}-\log\mathbf{T}^k_{i-3-j})/9 )
\end{equation}

\subsubsection{Scene expansion}
Due to camera movement, its field of view may extend into areas that have not yet been learned. Thus, an invisible mask \( M^{\text{ivsb}}_i \) is introduced to delineate these expansion areas. It is defined as the region where the rendered opacity exceeds a predefined threshold $\delta=0.8$. Once a sufficient amount of invisible areas is achieved, a scene expansion step is triggered to acquire additional Gaussians \( \mathcal{G}^{\text{add}}_i \) from the expansion areas: 
\begin{equation}
    \mathcal{G}^{\text{add}}_i=\mathbb{G}(M^{\text{ivsb}}_i \odot GRN(I_i,D_i),\mathbf{T}^k_i)
\end{equation}
The new Gaussians can then be obtained by merging $\mathcal{G}_{i-1}$ and $\mathcal{G}^{\text{add}}_i$.
\begin{equation}
    \mathcal{G}_i= \mathcal{G}_{i-1}\oplus \mathcal{G}^{\text{add}}_i
\end{equation}

\subsubsection{Deformation retrospective learning}
While the Gaussian deformation model is updated during the optimization of the camera pose, the achieved precision is insufficient for the demands of reconstruction. Unlike traditional SLAM systems that refine reconstruction based on key frames, our empirical findings indicate that dynamic scene learning necessitates a more thorough review of prior instances. Otherwise, in this sequential learning paradigm, deformations identified in later stages may inadvertently alter the earlier learning results. Consequently, we propose a deformation retrospective learning module that leverages a subset of past images to iteratively optimize the scene deformation. Specifically, during the $i^{\text{th}}$ learning cycle, following the scene expansion module, a training set comprising 40  frames is randomly sampled from a historical moment window $\{t_{j}|i-\omega< j\le i\}$ ($\omega$ is set to 100 in our work). The deformation module is then optimized on this set to integrate the historical deformation information.

\subsubsection{Multi-model representation}
%这里先说motivation
Inspired by the previous work~\cite{stilz2024flex}, a multi-model representation approach is implemented. It leverages multiple models to encode different temporal segments of the entire sequence. During the iterative frame-by-frame training process, once the current model encompasses a frame count exceeding a preset threshold \( \kappa=100 \), a new model instance is initiated on the new frame and trained following the procedure depicted in Fig.~\ref{fig:method}. This strategy prevents the issue of accumulating an excessive number of Gaussians, which could otherwise lead to substantial memory consumption and a consequent decrease in computational efficiency. By focusing on scene deformation within a confined temporal scope, each model simplifies the deformation learning challenge. Thanks to this, our approach is well-suited for the reconstruction of long video sequences.

\subsection{Generalizable Gaussian parameterization}
\label{sec:3.4}

\begin{figure}[tbh]
	\centering
	\includegraphics[width=0.43\textwidth]{figs/generalizable.pdf}
	\vspace{-3mm}
	\caption{Generalizable Gaussian parameterization module. The GRN is designed to predict pixel-aligned Gaussian attributes ($\alpha$, $\mathbf{s}$, $\mathbf{r}$) and correction terms ($\Delta D$, $\Delta C$) from the input frame consisting of a RGB image $I$ and a depth map $D$. These outputs are then utilized to construct a set of Gaussians on the camera coordinate system.} 
	\label{fig:generalizable}
 \vspace{-5mm}
\end{figure}
%这个是在整个framework哪一步？怎么又介绍回了GRN
In this section, we introduce the proposed Gaussian parameterization module, as illustrated in Fig. \ref{fig:generalizable}. Given a frame consisting of a RGB image $I \in \mathbb{R}^{H\times W\times 3}$ and a depth map $D \in \mathbb{R}^{H\times W}$, this module aims to generate well parameterized Gaussians in real-time from the pixels. A Unet-like Gaussian regressor network (GRN) is introduced to obtain Gaussian attributes from the input images. 

As stated before, each Gaussian has 5 properties the define its position, shape and appearance, i.e. $\mathcal{G}={\bm{\mu}, \mathbf{s}, \mathbf{r}, \mathbf{c}, \alpha}$. Previous methods often generate Gaussians from each pixels in the image and parameterize them with the pixel colors and depths directly. In this work, considering the limitation of reconstruction calculation and training time, only partial pixels in the image are involved by downsampling feature maps to reduce the size of Gaussians. This usually leads to inaccurate Gaussians representation when they are parameterized from the original pixel color and depth. To tackle this issue, we introduce the color correction term $\Delta C_x$ and depth correction term $\Delta D_x$ for a selected pixel with the image coordinate $x$, to xxxx 
Thus, we can obtain

\begin{align}
    \mathbf{c}&=SH(I_x+\Delta C_x)\\
    \bm{\mu}&=\Pi^{-1}(x, D_x+\Delta D_x)
\end{align}

where, $SH$ is the spherical harmonics converting function and $\Pi^{-1}$ symbolizes the inverse process of projection which transforms the image coordinates to the camera coordinates. 

% The GRN is expected to regress the correction terms $\Delta C$, $\Delta D$ and other attributes $\mathbf{s}$, $\mathbf{r}$, $\alpha$ from the given $I$ and $D$. It firstly generate the downsampled feature maps $\Gamma$ by convolutional layers and multiple prediction heads, each composed of two convolutional layers, are utilized to derive the Gaussian attributes from $\Gamma$. During module training, we used the identity matrix as the camera pose to render these parameterized Gaussians. The GRN is optimized to output reasonable Gaussian attributes and recover the original RGB image and depth map by rendering them.

The GRN aims to accurately predict the correction terms, \(\Delta C\) and \(\Delta D\), along with other attributes, \(\mathbf{s}\), \(\mathbf{r}\), and \(\alpha\), based on the input image \(I\) and depth map \(D\). The GRN is designed to extract some downsampled feature maps from the inputs and then predict Gaussian attributes from them by introducing multiple convolutional heads. During the training phase, this module is jointly trained with the Gaussian splatting architecture. The camera pose described with the identity matrix is utilized to render these parameterized Gaussians. The GRN is optimized to generate suitable Gaussian attributes and accurately recover the original RGB image and depth map through the rendering process.


%  \begin{align}
%     \Delta C &= HD_{\Delta C}(\Gamma)\\
%      \Delta D &= HD_{\Delta D}(\Gamma)\\
%      \mathbf{s} &= HD_{s}(\Gamma) \\
%      \mathbf{r} &= \mathbf{T}\cdot HD_{r}(\Gamma) \\
%      \alpha &= HD_\alpha(\Gamma)
%  \end{align}
 
% where, $HD_{\Delta C}$,  $HD_{\Delta D}$,$HD_{s}$, $HD_{r}$, $HD_{\alpha}$ represent the color correction head, the depth correction head, the scaling head, the rotation head, and the opacity head respectively.
     

\subsection{Gaussian deformation modeling}

\begin{figure}[tbh]
	\centering
	\includegraphics[width=0.43\textwidth]{figs/deformation.pdf}
	\vspace{-3mm}
	\caption{Illustration of the partial activated flexible Gaussian deformation model. Attributes of each Gaussian are defined by the deformation functions \( \Phi(t) \), which represent the deviation from the canonical values over time. This deformation function is articulated as a superposition of a series of Gaussian basis functions \( \{\varphi_j(t)\} \) and each is characterized by a triplet of parameters$\Theta_j=\{\tau_j,\sigma_j,w_j\}$. Only partial basis functions are activated and its parameters are optimized during training, while parameters of others are fixed.} 
	\label{fig:deformation}
\end{figure}



 In the context of surgical scene reconstruction, the complexity arises from tissue deformation due to breathing and instrument interactions, as well as variations in the observed color caused by the movement of light sources and changes in viewing angles. These factors render fixed Gaussian features insufficient for accurately describing such dynamic scenes.  Thus, as shown in Fig. \ref{fig:deformation}, our proposed method introduces a Gaussian deformation module and models the temporal evolution of Gaussian parameters as a function of time $t$, allowing the model to adapt and accurately represent the scene at each instant. Specifically, some additional parameters $\Theta_{\mu}$, $\Theta_{s}$, $\Theta_{r}$, $\Theta_{c}$ are learned to construct the deformation function $\Phi_{\mu}$, $\Phi_{s}$, $\Phi_{r}$, $\Phi_{c}$. Thus, the deformed Gaussian attributes can be obtained by adding the deformation $\Phi(t; \Theta)$ to the canonical values $\bm{\mu}_0$, $\mathbf{s}_0$, $\mathbf{r}_0$, and $\mathbf{c}_0$ which are derived from the generalizable Gaussian parameterization module.
 % \begin{align}
 %        \alpha(t) &= \alpha_0\\
 %     \bm{\mu}(t)&=\bm{\mu}_0+\Phi_{\mu}(t;\Theta_{\mu})\\
 %     \mathbf{s}(t)&=\mathbf{s}_0+\Phi_{s}(t;\Theta_{s}) \\
 %     \mathbf{r}(t)&=\mathbf{r}_0+\Phi_{r}(t;\Theta_{r}) \\
 %     \mathbf{c}(t)&=\mathbf{c}_0+\Phi_{c}(t;\Theta_{c})
 % \end{align}
% where, $\alpha_0$, $\bm{\mu}_0$, $\mathbf{s}_0$, $\mathbf{r}_0$, and $\mathbf{c}_0$ denote the canonical attributes which are derived from the generalizable Gaussian parameterization module.
 
The deformation function is defined as the sum of $B$ flexible basis functions $\Phi(t;\Theta)=\sum_{j=0}^B{ \varphi_j(t;\Theta_j)}$. (We set $B=20$ in this work.) The basis function is modeled as a Gaussian function, with its bias, shape, and size determined by a set of learnable parameters $\Theta_j=\{\tau_j,\sigma_j,w_j\}$. 
\begin{equation}
    \varphi_j(t;\Theta_j)=w_j\exp(-\frac{1}{2\sigma_j^2}(t-\tau_j)^2)
\end{equation}
For efficient learning, the initial biases $\tau^{\text{init}}_j$ are evenly spaced across the time span of the sequence and can be written as \( \tau^{\text{init}}_j = t_{\text{max}} \cdot j/(B - 1) \).

The deformation function leverages a natural advantage by decoupling deformations across different time points. This is due to the localized nature of the Gaussian basis function, which operates within a confined time span. In the context of the frame-by-frame sequential training approach explored in this paper, this characteristic effectively isolates the impact of the gradient learned in the current frame from previous deformations which is crucial for the overall reconstruction quality. 

However, a significant drawback is that each Gaussian needs to learn many additional parameters, which poses challenges to training efficiency and computing resources. Therefore, we introduce a partial basis function learning strategy in our approach. It can significantly reduce the number of parameters to be optimized in each iteration. Specifically, when learning the deformation at time $t$, only a subset of parameters $\{\Theta_j | t-t_{max}m/(B-1)<\tau^{init}_j<t+t_{max}m/(B-1)\}$ are optimized. The hyper-parameter $m$ is set to 4 here. 



\subsection{Loss functions}
We introduced three loss functions for the pre-training of GRN, as well as for the model training at stages of camera pose estimation and deformation retrospective learning. These functions aims to guide the rendered images and depth maps to closely approximate the original images and depth map ground truth.

When training GRN, the network is expected to recover the original input image and depth from the generated Gaussians.  L1 loss functions on the rendered RGB image $\hat{I}$ and depth map $\hat{D}$ were employed to optimize the predicted properties and correction terms for the generated pixel-aligned Gaussians.

\begin{equation}
    \mathcal{L}_{\text{g}}=\left | \hat{I}-I \right | + \lambda_\text{g}^\text{D}\left | \hat{D}-D \right | 
\end{equation}

During the camera pose estimation stage, completion of new scenes is not a desired goal and pixels within the region $M^{\text{ivsb}}$ are omitted from the loss calculation. Consistent with the methodologies of previous studies, a mask $M^{\text{ins}}$ that excludes the instrument was utilized to mitigate the occlusion effects caused by it. When evaluating on the Hamlyn dataset, due to the absence of the instrumental mask, a mask filled with ones was used instead. 

\begin{equation}
    \mathcal{L}_{\text{c}}=\left | M^{\text{c}}\odot(\hat{I}-I) \right | + \lambda_{\text{c}}^\text{D}\left |M^{\text{c}}\odot (\hat{D}-D) \right | + \lambda_{\text{c}}^{\text{r}}\Psi(\mathcal{G})
\end{equation}
where  $M^{\text{c}}=(1-M^{\text{ivsb}})\odot M^{\text{ins}}$, $\odot$ means the element-wise multiplication, and $\Psi(\mathcal{G})$ is a regularization term used to resist possible erroneous Gaussian displacements in scenes with camera motion. In this work, it is defined as the averaged movement of all Gaussians.
\begin{equation}
    \Psi(\mathcal{G})=\left \|\frac{1}{N}\sum_{n=1}^{N}{\bm{\mu}_n}\right \| ^2
\end{equation}
The loss utilized in the deformation learning stage is defined as
\begin{equation}
    \mathcal{L}_{\text{d}}=\left | M^{\text{ins}}\odot(\hat{I}-I) \right | + \lambda_{\text{d}}^\text{D}\left |M^{\text{ins}}\odot (\hat{D}-D) \right |
\end{equation}
The hyper parameters were set to $\lambda_\text{g}^\text{D}=0.002$, $\lambda_\text{c}^\text{D}=0.002$, $\lambda_\text{c}^\text{r}=0.01$, $\lambda_\text{d}^\text{D}=0.002$ respectively in this paper.

